On the Size Complexity of Non-Returning Context-Free PC Grammar Systems

Improving the previously known best bound, we show that any recursively enumerable language can be generated with a non-returning parallel communicating (PC) grammar system having six context-free components. We also present a non-returning universal PC grammar system generating unary languages, that is, a system where not only the number of components, but also the number of productions and the number of nonterminals are limited by certain constants, and these size parameters do not depend on the generated language.

==> dcfs.tex <==
\usepackage{amssymb,amsmath}
\makeatletter
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{definition}[theorem]{Definition\dromanb}
\newtheorem{remark}[theorem]{Remark\dromanb}
\newtheorem{example}[theorem]{Example\dromanb}
\newtheorem{claim}{\itshape Claim\d@cproof}
\newcommand*{\dromanb}{\gdef\d@tstyle{\rmfamily\upshape\mdseries}}

\newcommand{\d@tstyle}{}
\renewcommand{\@begintheorem}[2]{%
  \par\gdef\d@tstyle{\rmfamily\itshape\mdseries}\trivlist
  \item[\hskip\labelsep{\rmfamily\upshape\bfseries
    #1\ #2.}]\d@tstyle\ignorespaces}
\renewcommand{\@opargbegintheorem}[3]{%
  \par\gdef\d@tstyle{\rmfamily\itshape\mdseries}\trivlist
  \item[\hskip\labelsep{\rmfamily\upshape\bfseries
    #1\ #2\hskip\labelsep #3.}]\d@tstyle\ignorespaces}
\newcounter{d@proof}\let\thed@proof\relax\setcounter{d@proof}{0}
\newcommand*{\d@cproof}{%
  \ifnum \value{d@proof}=0{\@warning{\protect\begin{claim} ...
    \protect\end{claim} not nested in any `proof'^^J or `proofof'
    environment,}}\else\fi
}

%\newcommand*{\qed}{\raisebox{0.5ex}[0ex][0ex]{\framebox[1ex][l]{}}}
\newcommand*{\qed}{$\Box$}

\newenvironment{proof}{%
  \ifnum \value{d@proof}=0{\setcounter{claim}{0}}\else\fi
  \stepcounter{d@proof}\par\noindent
  {\rmfamily\itshape\mdseries Proof\/}:\hspace{\labelsep}\ignorespaces}%
  {\addtocounter{d@proof}{-1}\mbox{}\nolinebreak\hfill~%
  \ifnum \value{d@proof}=0{\qed}\else
    \ifnum \value{d@proof}=1{\qed\nolinebreak\,\nolinebreak\qed}\else
      \ifnum \value{d@proof}=2{\qed\nolinebreak\,\nolinebreak\qed
          \nolinebreak\,\nolinebreak\qed}\else
        {\qed\nolinebreak...\nolinebreak\qed}%
  \fi\fi\fi
  \medbreak
}
\newenvironment{proofof}[1]{%
  \vspace{\parskip}\vspace{\topsep}\vspace{\partopsep}%
  \ifnum \value{d@proof}=0{\setcounter{claim}{0}}\else\fi
  \stepcounter{d@proof}\par\noindent
  {\rmfamily\upshape\bfseries Proof of #1.}\hspace{\labelsep}\ignorespaces}%
  {\addtocounter{d@proof}{-1}\mbox{}\nolinebreak\hfill~%
  \ifnum \value{d@proof}=0{\qed}\else
    \ifnum \value{d@proof}=1{\qed\nolinebreak\,\nolinebreak\qed}\else
      \ifnum \value{d@proof}=2{\qed\nolinebreak\,\nolinebreak\qed
          \nolinebreak\,\nolinebreak\qed}\else
        {\qed\nolinebreak...\nolinebreak\qed}%
  \fi\fi\fi
  \medbreak
}
\newenvironment{proof*}{%
  \ifnum \value{d@proof}=0{\setcounter{claim}{0}}\else\fi
  \par\noindent
  {\rmfamily\itshape\mdseries Proof\/}:\hspace{\labelsep}\ignorespaces}%
  {
}
\makeatother

\setlength{\arraycolsep}{2.3pt}


==> eptcsdata.tex <==
\providecommand{\event}{J.~Dassow, G.~Pighizzini, B.~Truthe (Eds.): 11th International Workshop\\
on Descriptional Complexity of Formal Systems (DCFS 2009)}
\providecommand{\volume}{3}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{91}
\providecommand{\eid}{8}

